Abstraction Agent

Information abstraction, which groups strategically similar private states into a tractable number of buckets, is essential for scaling game-solving algorithms to large imperfect-information games. Constructing effective abstractions, however, has traditionally required domain-specific evaluators such as hand-strength calculators or equity estimators, which demand expert knowledge and engineering effort and are unavailable for most less-studied games. We propose the Abstraction Agent, a zero-shot pipeline that uses a large language model (LLM) to discover continuous strategic features from a natural-language game description, score private states on these features, and cluster them into abstraction buckets, without any game-specific evaluator, training data, or game-tree traversal during abstraction construction. The pipeline runs in four phases: feature discovery with calibration anchors, batched private-state scoring, correlation-based feature selection, and $k$-means clustering. The resulting abstractions reduce lifted-strategy exploitability by up to 62% relative to an expected-hand-strength baseline on heads-up no-limit Texas hold'em (HUNL) turn endgames, and beat a scalar rank baseline at every granularity on ROVER Trials, an original game absent from any pretraining corpus. Beyond these quantitative benchmarks, the pipeline transfers with unchanged prompts to four-card Pot-Limit Omaha, HUNL preflop and flop, and Riichi Mahjong, where the discovered features track each game's recognized strategic concepts. This is structured knowledge elicitation: converting implicit strategic knowledge in LLM parameters into explicit numerical features for downstream algorithmic computation. The code is available at https://github.com/lbn187/AbstractionAgent.

==> sections/limitations.tex <==
\section*{Limitations}

Our work has several limitations. First, the quantitative evaluation is limited to the two HUNL turn endgames that are publicly available from the Libratus subgame release, which form the complete public set of such turn subgames, and the original ROVER game, so broader validation across more game instances and game types remains future work. Second, the agent's advantage is strongest on streets with future cards; on the river, where EHS equals exact equity, multi-dimensional features provide limited additional benefit. Third, the method depends on the backbone's strategic knowledge: a frontier model (GPT-5.5) is needed to reliably beat EHS, whereas open-weight 32B/70B models are not competitive under the identical pipeline (Table~\ref{tab:backbone}); making the approach work with weaker or specialized backbones remains open. Relatedly, the advantage is granularity-dependent: at the coarse $K{=}20$ the agent underperforms EHS. Fourth, beyond the HUNL turn endgames and ROVER, the remaining cross-game results (PLO4, HUNL preflop/flop, Mahjong) are qualitative and assess strategic coherence rather than downstream exploitability. Fifth, while the pipeline avoids game-specific evaluators, it still requires a textual game description and rendering functions for private states, which presupposes some understanding of the game's structure.

\section*{Ethics Statement}

This work proposes a method for constructing information abstractions in imperfect-information games. The primary application domain is poker, which involves gambling. Although our experiments are research-oriented and evaluated on standard academic benchmarks (Libratus subgames), improved poker abstractions could in principle be used in automated gambling systems. We release code for reproducibility in controlled research settings but do not provide deployment tools for real-money play, and we encourage use only in academic contexts. The method itself is game-agnostic and has applications beyond gambling, including security games, negotiation, and multi-agent coordination.

\section*{Acknowledgments}

This work was supported by the National Natural Science Foundation of China Grant 52494974.

